Crowd Counting in Harsh Weather using Image Denoising with Pix2Pix GANs

Visual crowd counting estimates the density of the crowd using deep learning models such as convolution neural networks (CNNs). The performance of the model heavily relies on the quality of the training data that constitutes crowd images. In harsh weather such as fog, dust, and low light conditions, the inference performance may severely degrade on the noisy and blur images. In this paper, we propose the use of Pix2Pix generative adversarial network (GAN) to first denoise the crowd images prior to passing them to the counting model. A Pix2Pix network is trained using synthetic noisy images generated from original crowd images and then the pretrained generator is then used in the inference engine to estimate the crowd density in unseen, noisy crowd images. The performance is tested on JHU-Crowd dataset to validate the significance of the proposed method particularly when high reliability and accuracy are required.

==> figures/tab_counting.tex <==


% Table \ref{tab:counting}.
% \begin{table}[!h]
%     \centering
%     \setlength{\tabcolsep}{10pt}
%     \caption{Counting performance comparison of the proposed method over several baselines.} \label{tab:counting}
%     \begin{tabular}{r|c c c} \toprule
%     \textbf{Model}          &\textbf{GMAE(0)} &\textbf{GAME(1)} &\textbf{GAME(2)}  \\ \midrule
%     MCNN \cite{MCNN_CVPR2016}         &      &      &   \\ [0.3em]
%     MCNN \textbf{(ours)}    &      &      &       \\ [0.5em]
   
%     CSRNet \cite{CSRNet_CVPR2018}       &      &      &       \\ [0.3em]
%     CSRNet \textbf{(ours)}  &      &      &       \\ [0.5em]
    
%     TEDnet \cite{TEDnet_CVPR2019}       &      &      &       \\ [0.3em]
%     TEDnet \textbf{(ours)}  &      &      &       \\ [0.5em]
    
%     SASNet \cite{SASNet_AAAI2021}       &      &      &       \\ [0.3em]
%     SASNet \textbf{(ours)}  &      &      &       \\ [0.3em]
%     \bottomrule
%     \end{tabular}
% \end{table}

